Hardware Efficient Accelerator for Spiking Transformer With Reconfigurable Parallel Time Step Computing

This paper introduces the first low-power hardware accelerator for Spiking Transformers, an emerging alternative to traditional artificial neural networks. By modifying the base Spikformer model to use IAND instead of residual addition, the model exclusively utilizes spike computation. The hardware employs a fully parallel tick-batching dataflow and a time-step reconfigurable neuron architecture, addressing the delay and power challenges of multi-timestep processing in spiking neural networks. This approach processes outputs from all time steps in parallel, reducing computation delay and eliminating membrane memory, thereby lowering energy consumption. The accelerator supports 3x3 and 1x1 convolutions and matrix operations through vectorized processing, meeting model requirements. Implemented in TSMC's 28nm process, it achieves 3.456 TSOPS (tera spike operations per second) with a power efficiency of 38.334 TSOPS/W at 500MHz, using 198.46K logic gates and 139.25KB of SRAM.

==> Makefile <==
TARGET=main
LATEX_BUILD_CMD=xelatex -synctex=1 -shell-escape -interaction=nonstopmode

default: build

build:
	$(LATEX_BUILD_CMD) $(TARGET).tex
	bibtex main.aux || true
	$(LATEX_BUILD_CMD) $(TARGET).tex
	$(LATEX_BUILD_CMD) $(TARGET).tex | grep 'Warning\|pages'
clean:
	rm -rf *.aux *.log *.gz *.bbl *.blg *.lof *.lot *.toc *.out


==> ack/ack.tex <==
\begin{acknowledgement}%

在這兩年的碩士生涯中，我學會了如何深入探索和研究專業領域的知識，也讓自己在面對問題時能夠更加清晰地思考。實驗室的生活不僅教會了我如何與他人合作，也讓我學會了如何運用所學的知識來實現目標。

首先，我要感謝我的指導教授張添烜老師，老師在我的研究道路上就像一盞明燈，時常在我遇到困境時提點我，讓我不會迷失方向，在這兩年的學習過程中，老師給予我許多建議和研究上面的想法，對於我來說都十分重要。我也十分感謝黃俊達教授和劉靖家教授願意擔任我的口試委員。

同時，我也非常感謝實驗室的夥伴們，他們讓我的研究之旅充滿了歡笑和成長。在碩士一年級時，感謝洛亘、晏誠、姚遠、志嘉和子嘉的悉心指導；在過去的兩年裡，感謝民瀚、揚展、凱捷、奕萱、宗任、東軒、楚堯、芳淇、昶裕和慶林對我的幫助；在這一年裡，感謝宸瑜、崇維、瓊方、子源、豐賓和雨賢的陪伴。因為有你們的支持和陪伴，讓這段研究旅程變得更加有意義。

最後，我要感謝我的家人和女朋友瓊恩，是你們的支持讓我能夠順利完成學業，並繼續勇敢前行。







\end{acknowledgement}


==> thesis_new.tex <==
\ProvidesClass{thesis}[2022/02/25 V2.0]
\NeedsTeXFormat{LaTeX2e}


\DeclareOption*{\PassOptionsToClass{\CurrentOption}{book}}

\newif\ifTHESISOPTIONmaster         \THESISOPTIONmastertrue
\newif\ifTHESISOPTIONphd            \THESISOPTIONphdfalse

\DeclareOption{master}{\THESISOPTIONmastertrue\THESISOPTIONphdfalse}
\DeclareOption{phd}{\THESISOPTIONmasterfalse\THESISOPTIONphdtrue}

\newif\ifTHESISOPTIONen             \THESISOPTIONentrue
\newif\ifTHESISOPTIONzh             \THESISOPTIONzhfalse

\DeclareOption{en}{\THESISOPTIONentrue\THESISOPTIONzhfalse}
\DeclareOption{zh}{\THESISOPTIONenfalse\THESISOPTIONzhtrue}

\newif\ifTHESISOPTIONbinding      \THESISOPTIONbindingfalse
\DeclareOption{binding}{\THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONreview         \THESISOPTIONreviewfalse
\newif\ifTHESISOPTIONdraft          \THESISOPTIONdrafttrue
\newif\ifTHESISOPTIONfinal          \THESISOPTIONfinalfalse

\DeclareOption{review}{\THESISOPTIONreviewtrue
                       \THESISOPTIONdraftfalse
                       \THESISOPTIONfinalfalse
                       \THESISOPTIONbindingfalse}

\DeclareOption{draft}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdrafttrue
                      \THESISOPTIONfinalfalse
                      \THESISOPTIONbindingfalse}

\DeclareOption{final}{\THESISOPTIONreviewfalse
                      \THESISOPTIONdraftfalse
                      \THESISOPTIONfinaltrue
                      \THESISOPTIONbindingtrue}

\newif\ifTHESISOPTIONwatermark      \THESISOPTIONwatermarkfalse
\DeclareOption{watermark}{\THESISOPTIONwatermarktrue}

\ProcessOptions
\LoadClass[a4paper,12pt,oneside]{book}


\usepackage[BoldFont, SlantFont, CJKchecksingle, CJKmath=true]{xeCJK}
\usepackage{fontspec}     %
\usepackage{ifplatform}   %
\usepackage{indentfirst}  %
\usepackage{setspace}     %
\usepackage{tikz}         %
\usepackage{eso-pic}      %
\usepackage[xetex, hidelinks]{hyperref}  %
\usepackage{geometry}     %
\usepackage{emptypage}    %
\usepackage{afterpage}    %
\usepackage{lipsum}       %
\usepackage{verbatim}     %
\usepackage[retainorgcmds]{IEEEtrantools}  %
\usepackage{xCJKnumb}     %
\usepackage{titlesec}     %
\usepackage{titletoc}     %
\usepackage{tocloft}	  %
\usepackage{caption}	  %
\usepackage[labelformat=simple]{subcaption} %
\usepackage[chapter]{algorithm}  %


\ifTHESISOPTIONbinding  %
  \geometry{left=3 cm, right=2 cm, top=3 cm, bottom=3 cm}%
\else
  \geometry{left=2.5 cm, right=2.5 cm, top=3 cm, bottom=3 cm}%
\fi

\pagestyle{plain}
\setlength{\footskip}{1.5cm}

\doublespacing


\newcommand{\mainfont}[1]{%
\ifx&#1&%
  \setmainfont[Ligatures=TeX]{Times New Roman}
\else
  \setmainfont[Ligatures=TeX]{#1}
\fi
}

\newcommand{\sansfont}[1]{%
\ifx&#1&%
  \setsansfont[Ligatures=TeX]{Arial}
\else
  \setsansfont[Ligatures=TeX]{#1}
\fi
}


\newcommand{\mainfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKmainfont{DFKai-SB}  %
  \else\iflinux  %
    \setCJKmainfont{AR PL UKai TW}  %
  \else\ifmacosx  %
    \setCJKmainfont{Kaiti TC Regular}  %
  \else  %
    \setCJKmainfont{DFKai-SB}
  \fi\fi\fi
\else
  \setCJKmainfont{#1}
\fi
}

\newcommand{\sansfontzh}[1]{%
\ifx&#1&%
  \ifwindows  %
    \setCJKsansfont{PMingLiU}  %
  \else\iflinux  %
    \setCJKsansfont{AR PL UMing TW}  %
  \else\ifmacosx  %
    \setCJKsansfont{LiSong Pro}  %
  \else  %
    \setCJKsansfont{PMingLiU}
  \fi\fi\fi
\else
  \setCJKsansfont{#1}
\fi
}

\XeTeXlinebreaklocale "zh"
\XeTeXlinebreakskip = 0pt plus 1pt


\def\titlezh#1{\gdef\@titlezh{#1}}

\def\degreeyear#1{\gdef\@degreeyear{#1}}
\def\degreemonth#1{\gdef\@degreemonth{#1}}

\def\degreeyearzh#1{\gdef\@degreeyearzh{#1}}

\def\nation#1{\gdef\@nation{#1}}

\def\yearmonth#1{\gdef\@yearmonth{#1}}

\def\degree#1{\gdef\@degree{#1}}

\def\field#1{\gdef\@field{#1}}

\def\thesistype#1{\gdef\@thesistype{#1}}

\def\thesistypezh#1{\gdef\@thesistypezh{#1}}

\def\institute#1{\gdef\@institute{#1}}

\def\institutezh#1{\gdef\@institutezh{#1}}

\def\college#1{\gdef\@college{#1}}

\def\university#1{\gdef\@university{#1}}

\def\universityzh#1{\gdef\@universityzh{#1}}

\def\location#1{\gdef\@location{#1}}

\def\advisor#1{\gdef\@advisor{#1}}

\def\advisorzh#1{\gdef\@advisorzh{#1}}

\def\coadvisorA#1{\gdef\@coadvisorA{#1}}

\def\coadvisorAzh#1{\gdef\@coadvisorAzh{#1}}

\def\coadvisorB#1{\gdef\@coadvisorB{#1}}

\def\coadvisorBzh#1{\gdef\@coadvisorBzh{#1}}

\def\authorzh#1{\gdef\@authorzh{#1}}

\def\watermark#1{\gdef\@watermark{#1}}

\def\acktitle#1{\gdef\@acktitle{#1}}

\def\toctitle#1{\gdef\@toctitle{#1}}

\def\loftitle#1{\gdef\@loftitle{#1}}

\def\lottitle#1{\gdef\@lottitle{#1}}

\def\bibtitle#1{\gdef\@bibtitle{#1}}

\def\cvtitle#1{\gdef\@cvtitle{#1}}

\def\loptitle#1{\gdef\@loptitle{#1}}

\def\reservedfrontpages#1{\gdef\@reservedfrontpages{#1}}


\ifTHESISOPTIONmaster
  \thesistype{Master Thesis}%
  \thesistypezh{碩士論文}%
  \degree{Master}%
  \reservedfrontpages{0}%
\else
  \thesistype{Doctoral Dissertation}%
  \thesistypezh{博士論文}%
  \degree{Doctor of Philosophy}%
  \reservedfrontpages{0}%
\fi

\ifTHESISOPTIONzh
  \acktitle{誌謝}%
  \toctitle{目錄}%
  \loftitle{圖目錄}%
  \lottitle{表目錄}%
  \bibtitle{參考文獻}%
  \cvtitle{自傳}%
  \loptitle{著作目錄}%
\else
  \acktitle{Acknowledgement}%
  \toctitle{Table of Contents}%
  \loftitle{List of Figures}%
  \lottitle{List of Tables}%
  \ifTHESISOPTIONmaster
    \bibtitle{References}%
  \else
    \bibtitle{Bibliography}%
  \fi
  \cvtitle{Curriculum Vitae}%
  \loptitle{List of Publications}%
\fi


\renewcommand{\cfttoctitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftaftertoctitle}{\hspace*{\fill}}
\renewcommand{\cftlottitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterlottitle}{\hspace*{\fill}}
\renewcommand{\cftloftitlefont}{\hspace*{\fill}\Huge\bfseries}
\renewcommand{\cftafterloftitle}{\hspace*{\fill}}

\ifTHESISOPTIONzh
  \renewcommand{\contentsname}{\makebox[3em][s]{\@toctitle}}%
  \renewcommand{\listfigurename}{\makebox[4em][s]{\@loftitle}}%
  \renewcommand{\listtablename}{\makebox[4em][s]{\@lottitle}}%
  \renewcommand{\tablename}{表}%
  \renewcommand{\figurename}{圖}%
\else
  \renewcommand{\contentsname}{\@toctitle}%
  \renewcommand{\listfigurename}{\@loftitle}%
  \renewcommand{\listtablename}{\@lottitle}%
\fi

\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\xCJKnumber{\thecontentslabel}、\hspace{0.5em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries\makebox[1em][l]{\thecontentslabel}\hspace{0.25em}}{}%
  {\cftdotfill{\cftdotsep}\contentspage}%
\fi

\renewcommand\cftbeforetoctitleskip{-0.5cm}
\renewcommand\cftbeforeloftitleskip{-0.5cm}
\renewcommand\cftbeforelottitleskip{-0.5cm}

\def\maketocs{%
\ifTHESISOPTIONreview\else
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@toctitle}}%
  \tableofcontents
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@loftitle}}%
  \listoffigures
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@lottitle}}%
  \listoftables
\fi
}


\ifTHESISOPTIONzh
  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {\xCJKnumber{\thechapter}、\hspace{0.5em}}%
  {0em}{}%
\else
  \titleformat{\chapter}[display]%
  {\centering\Huge\bfseries}%
  {\chaptertitlename\ \thechapter}%
  {0em}{}%
\fi

\titlespacing*{\chapter}{0em}{-40pt}{*6}


\newcommand\BackgroundPicture{%
\ifTHESISOPTIONwatermark
  \ifTHESISOPTIONdraft
    \setlength{\@tempdimb}{.5\paperwidth}%
    \setlength{\@tempdimc}{.5\paperheight}%
    \setlength{\unitlength}{1pt}%
    \put(\strip@pt\@tempdimb,\strip@pt\@tempdimc){%
    \makebox(0,0){\rotatebox{45}{\textcolor[gray]{0.75}%
      {\fontsize{6cm}{6cm}\selectfont{DRAFT}}}}%
    }%
  \fi
  \ifTHESISOPTIONfinal
    \begin{tikzpicture}%
      \node[minimum width=\paperwidth,minimum height=\paperheight,opacity=0.75]%
        {\includegraphics[width=0.4\textwidth]{\@watermark}};%
    \end{tikzpicture}%
  \fi
\fi
}

\let\oldcleardoublepage\cleardoublepage
\renewcommand{\cleardoublepage}{%
  \newpage
  \ClearShipoutPicture
  \oldcleardoublepage
  \AddToShipoutPicture{\BackgroundPicture}%
}


\newcommand{\RNum}[1]{\uppercase\expandafter{\romannumeral #1\relax}}

\def\changemargin#1#2{\list{}{\rightmargin#2\leftmargin#1}\item[]}
\let\endchangemargin=\endlist 

\DeclareRobustCommand{\xCJKalphatozhnum}[1]{%
  \ifnum\strcmp{#1}{A} = 0 一 \else
  \ifnum\strcmp{#1}{B} = 0 二 \else
  \ifnum\strcmp{#1}{C} = 0 三 \else
  \ifnum\strcmp{#1}{D} = 0 四 \else
  \ifnum\strcmp{#1}{E} = 0 五 \else
  \ifnum\strcmp{#1}{F} = 0 六 \else
  \ifnum\strcmp{#1}{G} = 0 七 \else
  \ifnum\strcmp{#1}{H} = 0 八 \else
  \ifnum\strcmp{#1}{I} = 0 九 \else
  \ifnum\strcmp{#1}{J} = 0 十 \else
  \ifnum\strcmp{#1}{K} = 0 十一 \else
  \ifnum\strcmp{#1}{L} = 0 十二 \else
  \ifnum\strcmp{#1}{M} = 0 十三 \else
  \ifnum\strcmp{#1}{N} = 0 十四 \else
  \ifnum\strcmp{#1}{O} = 0 十五 \else
  \ifnum\strcmp{#1}{P} = 0 十六 \else
  \ifnum\strcmp{#1}{Q} = 0 十七 \else
  \ifnum\strcmp{#1}{R} = 0 十八 \else
  \ifnum\strcmp{#1}{S} = 0 十九 \else
  \ifnum\strcmp{#1}{T} = 0 二十 \else 零%
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
}


\newcommand{\addBibToContents}{%
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@bibtitle}}%
}

\renewcommand{\bibname}{\makebox[5.5em][s]{\@bibtitle}}


\renewcommand{\thealgorithm}{\arabic{chapter}.\arabic{algorithm}}


\newcommand{\addAppxToContents}{%
\addtocontents{toc}{\protect\setcounter{tocdepth}{0}}
\ifTHESISOPTIONzh
  \titlecontents{chapter}[0pt]{}%
  {\bfseries 附錄\xCJKalphatozhnum{\thecontentslabel}\quad}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%

  \titleformat{\chapter}[block]%
  {\centering\Huge\bfseries}%
  {附錄\xCJKalphatozhnum{\thechapter}\quad}%
  {0em}{}%
\else
  \titlecontents{chapter}[0pt]{}%
  {\bfseries \appendixname\hspace{0.5em}\thecontentslabel\hspace{0.5em}}%
  {}{\cftdotfill{\cftdotsep}\contentspage}%
\fi
}


\renewcommand\thesubfigure{ (\alph{subfigure})}


\def\coverpage
{
  \thispagestyle{empty}%
  \begin{center}
    \fontsize{18}{27}{\@universityzh}\\
    \fontsize{18}{27}{\@institutezh}\\
    \fontsize{18}{27}{\@thesistypezh}\\
    \ifTHESISOPTIONdraft
      \fontsize{18}{27}{初稿}\\
    \fi
    \vspace{2\baselineskip}
    
    \fontsize{14}{21}{\@institute}\\
    \fontsize{16}{24}{\@university}\\
    \fontsize{16}{24}{\@thesistype}\\
    \vspace{3\baselineskip} %

    \fontsize{18}{27}{\@titlezh}\\
    \vspace{0.75\baselineskip}
    \fontsize{18}{27}{\@title}\\
    \vspace{3\baselineskip} %
  
    \singlespacing
    \fontsize{18}{27}
    \begin{center}
    \begin{tabular}{c}%
      {研究生\ :} {\@authorzh \ (\@author)} \vspace{1em}\\%
      {指導教授\ :}{\@advisorzh \ (\@advisor)} \vspace{1em}\\%
      \ifx \@coadvisorAzh \@empty \else
        {\@coadvisorAzh(\@coadvisorA)} \vspace{1em}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        {\@coadvisorBzh(\@coadvisorB)} \vspace{1em}\\%
      \fi
    \end{tabular}%
    \end{center}
  \vspace{3cm}
  
  \fontsize{18}{27}\Large{\@nation} \Large{\@yearmonth}\\
  \LARGE{\@degreemonth} \ \LARGE{\@degreeyear} \\
  \end{center}
}


\def\titlepage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \begin{center}
    \singlespacing\Large
    \@titlezh\\
    \vspace{0.25\baselineskip}
    \@title\\
    \vspace{0.25\baselineskip}
  \end{center}
  \begin{flushleft}
    \singlespacing
    \setlength{\tabcolsep}{0.25em}
    \begin{tabular}{rl}%
      \large{\makebox[4em][s]{研究生}：}&\large{\@authorzh}\vspace{0.1em}\\%
      \large{指導教授：}&{\large{\@advisorzh}}\\%
      \ifx \@coadvisorAzh \@empty \else
        &{\large{\@coadvisorAzh}}\\%
      \fi
      \ifx \@coadvisorBzh \@empty \else
        &{\large{\@coadvisorBzh}}\\%
      \fi
    \end{tabular}%
    \hfill
    \begin{tabular}{ll}%
      \large{Student:}&{\large{\@author}}\vspace{0.5em}\\%
      \large{Advisor:}&{Dr. \large{\@advisor}}\\%
      \ifx \@coadvisorA \@empty \else
        &{\large{\@coadvisorA}}\\%
      \fi
      \ifx \@coadvisorB \@empty \else
        &{\large{\@coadvisorB}}\\%
      \fi
    \end{tabular}
  \end{flushleft}
  \vfill
  \begin{center}
    \large\@universityzh \vspace{-0.5em}\\
    \large\@institutezh \vspace{-0.5em}\\
    \ifTHESISOPTIONdraft
      \large\@thesistypezh \ 初稿\\
    \else
      \large\@thesistypezh\\
    \fi
    \vfill
    \ifTHESISOPTIONdraft
      \centerline{{A Thesis Draft}} \vspace{-1.0em}%
    \else
      \centerline{{A Thesis}} \vspace{-1.0em}%
    \fi
    Submitted to {\@institute} \vspace{-1.0em}\\
    \@college \vspace{-1.0em}\\
    \@university \vspace{-1.0em}\\
    in partial Fulfilment of the Requirements \vspace{-1.0em}\\
    for the Degree of \vspace{-1.0em}\\
    \@degree \vspace{-1.0em}\\
    in \vspace{-1.0em}\\
    \@field \vspace{-1.0em} \\
    \vspace{\baselineskip}
    \vfill
    {{\@degreemonth} {\@degreeyear}}\\
    \@location\\
    \vfill
    \Large{\@nation} \Large{\@yearmonth}
  \end{center}
}


\def\authzpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalzhpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\approvalenpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \phantomsection
  \null\newpage
}


\def\copyrightpage{
  \cleardoublepage
  \ClearShipoutPicture  %
  \thispagestyle{empty}
  \rule[0pt]{0pt}{0pt} \\
  \vspace{2.5in}
  \rule[0pt]{0pt}{0pt} \\
  \begin{center}
    \copyright {\@degreeyear} - {\@author}\\
    \vspace{0.5\baselineskip}
    All rights reserved.\\
  \end{center}
}


\def\maketitle{{
\ifTHESISOPTIONreview\else
  \coverpage


  \titlepage
  
  \input{ack/ack}
  

  \frontmatter
  


\fi
}}


\def\abszhpage
{
  \cleardoublepage
  \ifTHESISOPTIONfinal
    \setcounter{page}{\the\numexpr\@reservedfrontpages+\arabic{page}\relax}
  \fi
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{摘要}}
  \begin{center}
    \singlespacing
    {\Large \bf \@titlezh}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{學生：}&{\large{\@authorzh}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rlc}%
        \large{指導教授：}&{\large{\@advisorzh}}&{\large{博士}}\\%
        \ifx \@coadvisorAzh \@empty \else
          &{\large{\@coadvisorAzh}}&{\large{博士}}\\%
        \fi
        \ifx \@coadvisorBzh \@empty \else
          &{\large{\@coadvisorBzh}}&{\large{博士}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@universityzh\hspace{1ex}\@institutezh}\\
    \vspace{\baselineskip}
    \Large{\textbf{摘\qquad 要}}\\
  \end{center}
}

\newenvironment{abstractzh}{%
  \ifTHESISOPTIONreview\else
    \abszhpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\absenpage
{
  \cleardoublepage
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{Abstract}}
  \begin{center}
    \singlespacing
    {\Large \bf \@title}\\
    \vspace{\baselineskip}
    \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr}%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Student:}&{\large{\@author}}\\%
      \end{tabular}&%
      \setlength{\tabcolsep}{0.25em}%
      \begin{tabular}{rl}%
        \large{Advisor:}&{\large{Dr. \@advisor}}\\%
        \ifx \@coadvisorA \@empty \else
          &{\large{Dr. \@coadvisorA}}\\%
        \fi
        \ifx \@coadvisorB \@empty \else
          &{\large{Dr. \@coadvisorB}}\\%
        \fi
      \end{tabular}\\%
    \end{tabular*}\\
    \vspace{0.5\baselineskip}
    \large{\@institute}\\
    \large{\@university}\\
    \vspace{\baselineskip}
    \Large{\textbf{Abstract}}\\
  \end{center}
}

\newenvironment{abstract}{%
  \ifTHESISOPTIONreview\else
    \absenpage
    \par %
  \fi
  \ifTHESISOPTIONreview\comment\fi  %
}{%
  \ifTHESISOPTIONreview\endcomment\fi
}


\def\ackpage
{
  \cleardoublepage
  \ClearShipoutPicture  %
  \phantomsection
  \addcontentsline{toc}{chapter}{\textbf{\@acktitle}}
  \begin{center}
    \ifTHESISOPTIONzh
      {\LARGE \bf \makebox[3em][s]{\@acktitle}}\\
    \else
      {\LARGE \bf \@acktitle}\\
    \fi
  \end{center}
}

\newenvironment{acknowledgement}{%
  \ifTHESISOPTIONfinal
    \ackpage
    \par %
  \fi
  \ifTHESISOPTIONfinal\else\comment\fi  %
}{%
  \ifTHESISOPTIONfinal\else\endcomment\fi
}


\newenvironment{dedication}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \cleardoublepage
    \ClearShipoutPicture  %
    \thispagestyle{empty}%
    \vspace*{6.6cm}
    \begin{center}
  \fi\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\comment\fi\else\comment\fi
}{%
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd\else\endcomment\fi\else\endcomment\fi
  \ifTHESISOPTIONfinal\ifTHESISOPTIONphd
    \end{center}
  \fi\fi
}


\newenvironment{vita}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@cvtitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[3em][s]{\@cvtitle}}
    \else
      \chapter*{\@cvtitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}


\newenvironment{publications}{%
  \ifTHESISOPTIONreview\comment\else\ifTHESISOPTIONphd\else\comment\fi\fi
    \cleardoublepage
    \phantomsection
    \addcontentsline{toc}{chapter}{\textbf{\@loptitle}}
    \ifTHESISOPTIONzh
      \chapter*{\makebox[5.5em][s]{\@loptitle}}
    \else
      \chapter*{\@loptitle}
    \fi
}{%
  \ifTHESISOPTIONreview\endcomment\else\ifTHESISOPTIONphd\else\endcomment\fi\fi
}

\endinput

